Efficient Exact Algorithms for Maximum Balanced Biclique Search in Bipartite Graphs

Given a bipartite graph, the maximum balanced biclique (\textsf{MBB}) problem, discovering a mutually connected while equal-sized disjoint sets with the maximum cardinality, plays a significant role for mining the bipartite graph and has numerous applications. Despite the NP-hardness of the \textsf{MBB} problem, in this paper, we show that an exact \textsf{MBB} can be discovered extremely fast in bipartite graphs for real applications. We propose two exact algorithms dedicated for dense and sparse bipartite graphs respectively. For dense bipartite graphs, an $\mathcal{O}^{*}( 1.3803^{n})$ algorithm is proposed. This algorithm in fact can find an \textsf{MBB} in near polynomial time for dense bipartite graphs that are common for applications such as VLSI design. This is because, using our proposed novel techniques, the search can fast converge to sufficiently dense bipartite graphs which we prove to be polynomially solvable. For large sparse bipartite graphs typical for applications such as biological data analysis, an $\mathcal{O}^{*}( 1.3803^{\ddot{\delta}})$ algorithm is proposed, where $\ddot{\delta}$ is only a few hundreds for large sparse bipartite graphs with millions of vertices. The indispensible optimizations that lead to this time complexity are: we transform a large sparse bipartite graph into a limited number of dense subgraphs with size up to $\ddot{\delta}$ and then apply our proposed algorithm for dense bipartite graphs on each of the subgraphs. To further speed up this algorithm, tighter upper bounds, faster heuristics and effective reductions are proposed, allowing an \textsf{MBB} to be discovered within a few seconds for bipartite graphs with millions of vertices. Extensive experiments are conducted on synthetic and real large bipartite graphs to demonstrate the efficiency and effectiveness of our proposed algorithms and techniques.

==> deleted.tex <==
\iffalse


\noindent\textbf{One neighbour missing branching}. Let $u\in U(H)$ and $v\in V(H)$ be the pair of vertices missing one neighbour, and suppose $a-b\le \Delta$, we propose the following reduction rule.
\begin{lemma}
 Let $u\in U(H)$ and $v\in V(H)$ be the pair of vertices missing one neighbour, remove both $u$ and $v$, and create two branches for solving $(a-1,b)$ and $(a, b-1)$ balanced biclique problem.
%decrease $\Delta$ by $1$
\end{lemma}
\noindent\textbf{Two neighbours missing branching}. Let $u\in U(H)$ be the vertex connecting to every vertex in $V(H)$ expect for $v$ and $w$, and suppose $a-b-1\le \Delta$, we propose the following reduction rule.
\begin{lemma}
\begin{itemize}
  \item if $N(v)==N(w)$, remove $u$, $v$ and $w$, and create two branches for solving $(a-1,b)$ and $(a,b-2)$ balanced biclique problems by selecting $u$ or $\{v,w\}$ respectively .
  \item if $N(V)\cap N(w)=\emptyset$, remove $u,v,w$ and create three branches $(a-1, b)$, $(a, b-1)$, $(a, b-1)$ balanced biclique problems by selecting $u$, $v$ or $w$ respectively.
\end{itemize}
\end{lemma}
%depends on the common neighbours


\textit{One neighbour missing reduction:} need proof

\textit{Two neighbour missing reduction:} need proof

\textit{Three neighbour missing reduction:} need proof










\noindent\textbf{Efficient implementation of reductions}. Algorithm, correctness proof and time complexity analysis.



\noindent\textbf{Heuristics for enumeration}.



\begin{problem*}\label{p:2}  \textup{\textbf{Finding maximum edge $\delta$-balanced biclique}}
Given a bipartite graph $G=$($U,V,E$), and an integer $\Delta$, find a $\delta$-balanced biclique $(A,B)$ such that there is no $C'$ any other $\Delta$-balanced bilcique $(A',B')$ such that $|A'|\times|B'|> |A|\times|B|$.
\end{problem*}
\fi

\iffalse
\subsection{Sampling algorithm for finding ($\rho,\Delta$) balanced biclique }



\noindent\textbf{High level idea}.
\begin{enumerate}
  \item Select a random subset $S$ of size $x$ uniformly from the set of columns $\{1,2,\ldots,|V(g)|\}$. Assuming $S\cap C^{*}\ne \emptyset$.

  \item Select the edges ($E'$) that appear exactly $r^{*}$ times in the rows of $X_{[1:v(G],S\cap C^{*}}$.
  \item Set $R^{*}$ to be the set of rows in which $E'$ appear.
  \item Set $C^{*}$ to be the set of clean columns corresponding to $R^{*}$.
\end{enumerate}


\noindent\textbf{Parameters}
\begin{enumerate}
  \item $t$: number of iterations
  \item $x$: projection size
  \item $x_{min}$: the size of the smallest subset of the projection
  \item $c$, $r$: the thresholds on the number of columns and rows
\end{enumerate}



\subsection{Search order and upper bound for MDBBC Search}
\subsection{Upper bounds and search orders}
The first upper bound which we consider is based on the definition of coreness, or equivalently degeneracy.

We firstly revisit the definition of degeneracy.

\noindent\textbf{Core based degeneracy order}. The degeneracy of graph $G$, is the smallest integer $k$, such that the vertices of $G$ can be arranged in a permutation so that each vertex is adjacent to at most $k$ of the vertices in the graph that is induced by its following vertices. The degeneracy of graph $G$ has a symbol of $\delta$($G$).

We propose bitrussness based degeneracy order as following.

\noindent\textbf{Butterfly and bitrussness}.

\noindent\textbf{Bitrussness based degeneracy order}. The bitrussness based degeneracy of graph $G$, is the smallest integer $\phi$, such that the edges of $G$ can be arranged in a permutation so that each edge is butterfly adjacent to at most $\phi$ of the edges in the graph that is induced by its following edges. The bitrussness based degeneracy of graph $G$ has a symbol of $\Phi$($G$).

%Next, we shall have several reductions, proving that \textsc{Problem}~\ref{p:1} is W[1]-hard on condition that the degeneracy of $G$ is small, i.e., $G$ is a sparse graph.







%\subsection{Transform maximum balanced clique problem to ($\rho,\Delta$) balanced biclique problems}


%\noindent\textbf{Vertex ego subgraph based on core degeneracy order}



%\noindent\textbf{Edge ego subgraph based on bitrussness degeneracy order}



%\noindent\textbf{The size of the ego subgraphs are small}. A lemma and proof.



%\noindent\textbf{The ego subgraphs are dense}. A lemma and proof.



%\noindent\textbf{Compact and effective data structure storing ego subgraphs}. Store the subgraph as adjacency matrix.

\subsection{Exact algorithm for finding ($\rho,\Delta$) balanced biclique }

\noindent\textbf{Notations}:
\begin{enumerate}
  \item $g$: a small, connected and dense bipartite subgraph
  \item $d(u,g)$: degree of $u$ in subgraph $g$

\end{enumerate}


\noindent\textbf{Novel enumeration algorithm}.

\begin{algorithm}
    \KwIn{$(U,V,E)$}
    \KwOut{}

    $(R_{U}, R_{V})$ $\leftarrow$ $(\emptyset, \emptyset)$\;
    $(P_{U}, P_{V})$ $\leftarrow$ $(U,V)$\;
    $(X_{U}, X_{V})$ $\leftarrow$ $(\emptyset, \emptyset)$\;

    \SetKwProg{myproc}{Procedure}{}{}
    \SetKwFunction{proc}{proc}
    \myproc{\proc{}}{

    }


\end{algorithm}

\subsection{References}
Generated by bibtex from your ~.bib file.  Run latex,
then bibtex, then latex twice (to resolve references).

%APPENDIX is optional.
% ****************** APPENDIX **************************************
% Example of an appendix; typically would start on a new page
%pagebreak

\begin{appendix}
You can use an appendix for optional proofs or details of your evaluation which are not absolutely necessary to the core understanding of your paper.

\section{Final Thoughts on Good Layout}
Please use readable font sizes in the figures and graphs. Avoid tempering with the correct border values, and the spacing (and format) of both text and captions of the PVLDB format (e.g. captions are bold).

At the end, please check for an overall pleasant layout, e.g. by ensuring a readable and logical positioning of any floating figures and tables. Please also check for any line overflows, which are only allowed in extraordinary circumstances (such as wide formulas or URLs where a line wrap would be counterintuitive).

Use the \texttt{balance} package together with a \texttt{\char'134 balance} command at the end of your document to ensure that the last page has balanced (i.e. same length) columns.

\end{appendix}
\fi

%We observed that given a large and sparse bipartite graph $G$, we can partition $G$ into fixed number of compact and dense subgraphs.
%When evaluating each small while dense subgraphs, we can apply easy implementable, low cost, but effective simplification rules, to reduce the difficulty of exhaustive search as much as possible.
%Further more, it is also possible to estimate the upper bound size of $\delta$ balanced biclique for each of the subgraphs.
%As such, we can evaluate each of the subgraphs in an order according to their upper bound sizes.
%Following such order, we can heuristically find a large size $\delta$ balanced biclique and have high chance to avoid evaluate all the subgraphs.





%We observed that given a vertex $u$ in a bipartite graph $G$, the maximum $\delta$ balanced biclique that involves $u$ can be restricted to a small subgraph (will be introduced later), and at the same time the upper bound size of $\delta$ balanced biclique contained by the small subgraph can be estimated reasonably.
%As such, using the upper bound size as a fixed parameter, say, $\rho$, we can perform ($\rho$,$\delta$) balanced clique search in the small subgraph.

%With this idea, we order vertices of $G$ according to the upper bound size of the $\delta$ balanced bicliques that each vertex can involved.
%Then we perform fixed parameter search for each vertex in its restricted small subgraph.
%As such, we can derive large size $\delta$ balanced biclique early and have chance to avoid to explore every vertex. 
